GenMix: Combining Generative and Mixture Data Augmentation for Medical Image Classification

In this paper, we propose a novel data augmentation technique called GenMix, which combines generative and mixture approaches to leverage the strengths of both methods. While generative models excel at creating new data patterns, they face challenges such as mode collapse in GANs and difficulties in training diffusion models, especially with limited medical imaging data. On the other hand, mixture models enhance class boundary regions but tend to favor the major class in scenarios with class imbalance. To address these limitations, GenMix integrates both approaches to complement each other. GenMix operates in two stages: (1) training a generative model to produce synthetic images, and (2) performing mixup between synthetic and real data. This process improves the quality and diversity of synthetic data while simultaneously benefiting from the new pattern learning of generative models and the boundary enhancement of mixture models. We validate the effectiveness of our method on the task of classifying focal liver lesions (FLLs) in CT images. Our results demonstrate that GenMix enhances the performance of various generative models, including DCGAN, StyleGAN, Textual Inversion, and Diffusion Models. Notably, the proposed method with Textual Inversion outperforms other methods without fine-tuning diffusion model on the FLL dataset.

==> sections/2_relatedworks.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Section 2: Related Works %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Works}
\label{sec:related}

%%%%% Section 2.1: Generative Models for Data Augmentation %
\subsection{Generative Models for Data Augmentation}




%%%%% Section 2.2: Mixture Data Augmentation Models %%%%%%%%
\subsection{Mixture Data Augmentation Models}



==> sections/5_discussions.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Section 5: Discussions %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Discussions}
\label{SEC:DISCUSSIONS}

% P1: 요약, 실험결과, 향후 과제
In this paper, we introduced GenMix, a novel data augmentation method based on the diffusion model for the classification of FLLs in CT images.
The proposed method generates synthetic images of FLLs from a pre-trained diffusion model without additional training by utilizing the Textual Inversion technique.
Additionally, it utilizes MixUp between the real and mixed data to enhance the quality of the synthetic images and strengthen the boundary between classes.
In experiments, the proposed method significantly improved the classification performance of diffusion model-based data augmentation through MixUp.
Furthermore, GenMix outperformed the fine-tuned StyleGAN-based data augmentation, even without additional training of the diffusion model.
% Future research will include (1) further improving the quality of synthetic image generation by replacing the natural image-trained diffusion model in Textual Inversion with a medical image-pre-trained diffusion model, and (2) validating the generalizability of GenMix by applying it to other image classification tasks.

